Sparse and Privacy-enhanced Representation for Human Pose Estimation

We propose a sparse and privacy-enhanced representation for Human Pose Estimation (HPE). Given a perspective camera, we use a proprietary motion vector sensor(MVS) to extract an edge image and a two-directional motion vector image at each time frame. Both edge and motion vector images are sparse and contain much less information (i.e., enhancing human privacy). We advocate that edge information is essential for HPE, and motion vectors complement edge information during fast movements. We propose a fusion network leveraging recent advances in sparse convolution used typically for 3D voxels to efficiently process our proposed sparse representation, which achieves about 13x speed-up and 96% reduction in FLOPs. We collect an in-house edge and motion vector dataset with 16 types of actions by 40 users using the proprietary MVS. Our method outperforms individual modalities using only edge or motion vector images. Finally, we validate the privacy-enhanced quality of our sparse representation through face recognition on CelebA (a large face dataset) and a user study on our in-house dataset.

==> fig/fig_env.tex <==

% \begin{figure}[H]
%     \centering
%     \vspace{-0.35cm}
%     % \subfiguretopskip=2pt    
%     % \subfigurebottomskip=2pt    
%     % \subfigurecapskip=2pt    
%     \subfigure[]{
%     \label{fig:env_pic}
%     \includegraphics[width=0.4\linewidth]{src/env.pdf}}
%     \quad
%     \subfigure[]{
%     \label{fig:env_draw}
%     \includegraphics[width=0.4\linewidth]{src/env_draw.pdf}}
%     \caption{(a) Our dataset is collected in a room with the area 6$\times$5m$^{2}$. (b) Two MVSs are placed 3 meters away from the subject. MVS 1 is placed directly facing the participant and MVS 2 is placed at the viewing angle of 45 degrees.}
%     \label{fig:env}
% \end{figure}


\begin{figure}
  \begin{minipage}[c]{0.45\textwidth}
    \includegraphics[width=\textwidth]{src/env_draw.pdf}
    \vspace{-2\baselineskip}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.5\textwidth}
    \caption{
       Two MVSs are placed 3 meters away from the subject, with a viewing angle of 45 degrees centered on the subject's position.
    } \label{fig:env}
  \end{minipage}
\end{figure}


% \begin{wrapfigure}{r}
%     \centering
%     {\includegraphics[width = 0.48\linewidth]{src/env_draw.pdf}}
%     \caption{Two MVSs are placed 3 meters away from the subject, with a viewing angle of 45 degrees centered on the subject's position.}

%     \label{fig:env_wrap}
% \end{wrapfigure}

==> fig/fig_fusion.tex <==
% \begin{figure}[ht]
%     \centering
%     {\includegraphics[width = 0.5\linewidth]{src/early fusion3d.pdf}}
%     \caption{Fusion model. We perform early fusion on different modalities of data, including edge image and 2-directional motion vectors, where the output channel N is the number of joints.}
%     \label{fig:fusion}
% \end{figure}



\begin{figure}
\hspace{0.2cm}
  \begin{minipage}[c]{0.45\textwidth}
    \includegraphics[width=\textwidth]{src/early fusion3d.pdf}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.45\textwidth}
    \caption{
       Fusion model. We perform early fusion on different modalities of data, including edge and 2-directional motion vectors, where the output channel $N$ is the number of joints.
    } \label{fig:fusion}
  \end{minipage}
\end{figure}

==> fig/fig_fusion_new.tex <==
\begin{wrapfigure}{r}[0.1cm]
    \centering
    {\includegraphics[width = 0.48\linewidth]{src/early fusion3d.pdf}}
    \caption{Fusion model. We perform early fusion on different modalities of data, including edge image and 2-directional motion vectors, where the output channel N is the number of joints.}

    \label{fig:fusion}
\end{wrapfigure}

==> fig/fig_qual.tex <==
\begin{figure*}[ht]
    \centering
    {\includegraphics[width = 1\linewidth]{src/qual_sim.pdf}}
    \caption{Qualitative results. Each row contains 4 modalities of input data and 2 predicted results: the first predicted result is based on the edge input only, and the second is based on the fusion of the edge and motion inputs. The input data modalities are grayscale image, edge image, horizontal motion vector, and vertical motion vector. The red dots indicate the predicted keypoints, and the green ones indicate the ground truth.}
    \label{fig:qual}
\end{figure*}

==> fig/fig_recognition.tex <==
% \begin{figure}[ht]
%     \centering
%     {\includegraphics[width = 1\linewidth]{src/ROC.pdf}}
%     \caption{ROC curves for face recognition.  We use ArcFace model training on different modality of data. During training on motion vector data, we additionally filter out images with insufficient effective values to enhance the training. However, this filtering process is not necessary for grayscale, edge, and fusion training}
%     \label{fig:roc}
% \end{figure}

==> tab/tab_keypoints_speed.tex <==
% Table generated by Excel2LaTeX from sheet '工作表1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|cccccc}
    \hline
    Keypoint & \multicolumn{2}{c}{\# of Slow Motions} & \multicolumn{2}{c}{\# of Medium Motions} & \multicolumn{2}{c}{\# of Fast Motions} \bigstrut\\
    \hline
    Nose  & \multicolumn{2}{c}{151909} & \multicolumn{2}{c}{24880} & \multicolumn{2}{c}{15211} \bigstrut[t]\\
    Shoulder (R/L) & 153705 & 154281 & 22587 & 21815 & 15708 & 15904 \\
    Elbow (R/L) & 130450 & 142771 & 33854 & 25689 & 27696 & 23540 \\
    Hip (R/L) & 154352 & 154678 & 22757 & 22501 & 14891 & 14821 \\
    Hand (R/L) & 109474 & 134175 & 39823 & 26796 & 42703 & 31029 \\
    Knee (R/L) & 143297 & 148686 & 29046 & 25024 & 19657 & 18290 \\
    Foot(R/L) & 143297 & \textcolor[rgb]{ .122,  .122,  .122}{148686} & 29046 & 25024 & 18290 & \textcolor[rgb]{ .122,  .122,  .122}{20472} \\
    Total & \multicolumn{2}{c}{1881037} & \multicolumn{2}{c}{338077} & \multicolumn{2}{c}{276886} \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

